Cube Interestingness: Novelty, Relevance, Peculiarity and Surprise

In this paper, we discuss methods to assess the interestingness of a query in an environment of data cubes. We assume a hierarchical multidimensional database, storing data cubes and level hierarchies. We start with a comprehensive review of related work in the fields of studies of human behavior and computer science. We define the interestingness of a query as a vector of scores along difference dimensions, like novelty, relevance, surprise and peculiarity and complement this definition with a taxonomy of the information that can be used to assess each of these dimensions of interestingness. We provide both syntactic (result-independent) checks and extensional (result-dependent) measures and algorithms for assessing the different dimensions of interestingness in a quantitative fashion. We also report our findings on a user study that we conducted, analyzing the significance of each dimension, its evolution over time and the behavior of the study's participants.

==> 100_DraftLeftOvers.tex <==
% !TeX spellcheck = en_US
\section{REMOVED FROM MAIN TEXT}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\isDraft{

\subsection{Relevance: Family-based relevance, or, relevance based on structural ties and not areas of interest [DRAFT]}\label{section:_2kk65je17ecg}

So far, the intuition behind the notion of relevance has been based on queries exploring smaller parts of a larger subset of the multidimensional space (the analyst's goal) from different, complementary angles, in terms of selection filters, levels of grouping and potentially measures and aggregation functions (remember that the latter do not play a role in the evaluation of relevance).

What if the basis of relevance is not defined by the underlying area of interest, but with respect to the structural similarity of the involved queries? As we will see right away, there are several ways that can make two queries be semantically related (equivalently, "relevant"), based on the commonality of a subset of their definition rather than a pre-defined user area of interest.

%KILLED, not valid, left as a remnant of a nice idea
%Thus, in the sequel, we define a query as being relevant to its \textit{previous one} (and not the previous history) on the basis of structural similarity.\footnote{This can indeed be viewed as a special case of a history with just one query, the previous, or a very specific goal defined as a query rather than just a selection predicate. Also, although combinations of the categories can be envisioned, we will remain within the scope of relevance evaluation with respect to a single predecessor query.} Moreover, 

In our discussion, we will focus on "family-ties" i.e., query similarity on the basis of the relationship of values and levels participating in the two involved queries.

Specifically, given a specific query $q$, we define as \textit{family-related} queries, the following classes of queries 
the following classes of queries:

\begin{itemize}
\item \textit{siblings(q)}, i.e., queries identical to $q$ 
with a single exception: instead of an atom \textit{Level = value}, each $q_{i}$ in \textit{siblings(q)} has an atom. 
\textit{Level=u}, $u$ in \textit{siblings(value)}, with \textit{siblings(value)} being all the values having the same direct ancestor with \textit{value}.
\item \textit{children(q)}, as above, but with the values in the immediate descendants of \textit{value}.
\item \textit{mother}(\textit{q}), as above, but with $u$ being the immediate ancestor of \textit{value}.
\item \textit{ancestor}($q$ at level $L'$) or \textit{descendant}($q$ at level $L'$) similarly.
\item \textit{pastVersions(q,k)}, which means that the 
query $q$ involves a time-related dimension, and an atom \textit{TimeLevel = value}, and we take the $k$ previous 
values of \textit{value} (almost similar to siblings, although the $k$ past values are not necessarily siblings of \textit{value}).
\item \textit{measureSibling(q, M, M')}, i.e., a query identical to $q$ with a single exception: another measure $M'$, instead of $q.M$.
\end{itemize}


\emph{Assuming now that a query $q^{n}$ ("n" for new) is assessed with respect to a query $q^{o}$ ("o" for old), belonging to one of the above categories, how are we to assess relevance of the two family-related queries}? \\

\textbf{Boolean result}. The easiest way to assess structural relevance is via a Boolean decision, on whether $q^{n}$ belongs to one of the categories that make it eligible for structurally relevant. In measurable fashion, the distance is 1 if the new query is structurally irrelevant, or, 0 if relevant. \rem{Spyros' algo Family-based 3.1.2.1b}\\

\textbf{Peculiarity Score}. As we detail in Section~\ref{sec:peculiarity}, we can measure the distance of two queries in various ways, including the cases: (i) before executing queries and without the presence of results, and, (ii) after query execution, on the basis of the similarity of their cells. We refer the reader to  Section~\ref{sec:peculiarity} on how this is doable.

Moreover, assuming a list of queries $Q$ (either a query session or query history) and a new query $q$, we can compute the average/max/min distance of $q$ to the queries of $Q$ as a measure of its relevance. \\

\textbf{Age-based Score}. Assume $q^{k+1}$ is the new query and $Q$ is the list of $k$ previous queries. We can combine the above measurements orthogonally to an aging factor, that shows how far back in the history is each query $q^i$ in $Q$ compared to the new $q^{k+1}$. Thus, we orthogonally assume a $dist(\cdot)$ function as one of the aforementioned distance functions and compute 
\[
dist^{age}(q^{k+1},q^i) = e^{-\alpha \cdot {(k+1-i)}^{-1}} \cdot dist(q^{k+1},q^i), \alpha > 0
\]

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{media/agingFactor}
\caption{Reminder of aging factors.}\label{fig:aging}
\end{figure}

The overall relevance value of $q^{k+1}$ with respect to $Q$ can again be computed as the last (i.e., against the last query $q^k$), average, max, min, or other aggregate value over the members of $Q$.\\




\hrulefill

\textbf{Query Category as an assessor of relevance}.\inlineRem{DRAFT} What if we do not compute $relevance(q^n,q^o)$ but we measure $relevance(q^n,q^o~|~q^{n}.type)$, the query type explaining what kind of intentional query $q^n$ is (e.g., describe, assess, explain, etc). We will refer to the query type as the query goal $q.goal$, henceforth, as the intention of the user characterizes whether the goal involves a simple description, a prediction, explanation etc..

Then, we can assign a weight to the relevance, depending on a \textit{distance score} between the above categories and a specified query goal. I.e., $relevance(q' | q.g) = score(q'.category~wrt~to~q~|~
q.goal)$\\

For example, we can have:

\begin{itemize}
\item \textit{score(siblings, assess) = 90\%}
\item \textit{score(any other of the above, assess) = 7\%}
\item \textit{score(none of the above, assess) = 3\%}
\end{itemize}






Then, if a query $q^n$ belongs to siblings of $q^o$, its relevance is 90\%.


} % end isDraft
% %%%%%%%%%%%%% END IS DRAFT %%%%%%%%%%%%%%%%%%%

\hrulefill

%%%%%% IS DRAFT
\isDraft{
\subsection{Peculiarity: Other considerations for automatically computing cell 
mappings [DRAFT, OPEN, F.W.]}\label{section:_op3m44afi4cr}

\inlineRem{DRAFT: probably FUTURE WORK}

\subsubsection{from outlierness definition}
Apart from kNN, can also check for outliers in document mining, since each document is a bag of words, and here we want to compute the distance of two \underline{sets} of cells. See aggarwal at SDM'17 as the latest I have found.





\subsubsection{measure comparison}

All the previous measures are oriented towards the \textit{coordinates} of the cells. At the end of the day, what is actually measured by query peculiarity is mostly on whether the query definition locates it  in an area of the multidimensional space that is infrequently visited by 
other queries.

\textit{What if I want to compare the measures of the cells of the 
query results to the respective measures of the cells of other queries?
}

\hrulefill

For example, assume the 

\begin{itemize}
\item grouper set \{product, store\} and the filters city=Athens, 
year=2020
\item a set of queries that are identical with the exception of year, 
e.g., year = 2019, year = 2018, ...
\end{itemize}
(i.e., you have the same city and you measure sum(sales) per product, 
store for different years).

How can I measure outlierness?

\hrulefill

Peculiarity should probably be more related to explain + 
describe(practically, describe carries no semantics=$>$ "\,blind 
measures like novelty and peculiarity are most appropriate for 
describe\ldots )

--------------------



Must / can devise an algo where

Foreach cell c in q.result\{

Detect one cell from each query of the query set s.t., they all belong 
to the same equivalence class (e.g., with the exception of one 
dimension, say D, all other coordinates are the same, and for D, the 
values are siblings);

Check whether c.M is an outlier;

\}

q.outliernessScore = Count how many/what percentage of cells of q are 
outliers

----------



For the above necessary conditions needed. Assume all queries have:

\begin{itemize}
\item All queries have the same \textbf{A}.
\item $\phi$  = conjunction of atoms, all atoms of the form D.L=value
\item All queries have the same atoms except for a single dimension D, 
s.t., D not in \textbf{A}.
\begin{itemize}
\item Each query has an atom D.L=value, all queries have the same L for 
each selection atom (i.e., the filter either the same member or 
same-level members).
\end{itemize}
\end{itemize}
Then, you map by coordinates, excluding D.

Can we do the same exercise with a cube's ancestor / children? The above 
is practically comparing a cube to its siblings.

} %isDraft
% %%%%%%%%%%%%%%%% END ISDRAFT
